Exponential Quantum Speedup for Simulation-Based Optimization Applications

The simulation of many industrially relevant physical processes can be executed up to exponentially faster using quantum algorithms. However, this speedup can only be leveraged if the data input and output of the simulation can be implemented efficiently. While we show that recent advancements for optimal state preparation can effectively solve the problem of data input at a moderate cost of ancillary qubits in many cases, the output problem can provably not be solved efficiently in general. By acknowledging that many simulation problems arise only as a subproblem of a larger optimization problem in many practical applications however, we identify and define a class of practically relevant problems that does not suffer from the output problem: Quantum Simulation-based Optimization (QuSO). QuSO represents optimization problems whose objective function and/or constraints depend on summary statistic information on the result of a simulation, i.e., information that can be efficiently extracted from a quantum state vector. In this article, we focus on the LinQuSO subclass of QuSO, which is characterized by the linearity of the simulation problem, i.e., the simulation problem can be formulated as a system of linear equations. By cleverly combining the quantum singular value transformation (QSVT) with the quantum approximate optimization algorithm (QAOA), we prove that a large subgroup of LinQuSO problems can be solved with up to exponential quantum speedups with regards to their simulation component. Finally, we present two practically relevant use cases that fall within this subgroup of QuSO problems.

==> tikz/quso-old.tex <==
\begin{quantikz}[column sep=7pt, row sep={10pt}]
\lstick{$\ket{0}^{\otimes n}$} & \gate{H^{\otimes n}} & \gate[5][2.4cm]{U_f}\gateinput[1]{$x$}\gateoutput[1]{$x$}\gategroup[5,steps=3,style={inner xsep=0pt, fill=blue!20},background,label style={label position=above,anchor=south, yshift=-0.8mm}]{$U_C(\gamma_1)$} & \qw & \gate[5]{U^\dagger_f} & \midstick[1]{$e^{-i \gamma_1 f(x)}\ket{x}$} & \gate{U_M(\beta_1)} & \ \ldots\ & \gate[5]{U_C(\gamma_p)} & \gate{U_M(\beta_p)} & \meter{} \\
\lstick[3]{$\ket{0}^{\otimes m}$} & \qw & \gateinput[3]{$0$}\gateoutput[3]{$f(x)$} & \gate{P(-\frac{\gamma_1}{2^{1}})} & \qw & \midstick[3]{$\,\ket{0}^{\otimes m}\,$} & \qw & \ \ldots\ & \qw & \qw &  \rstick[3]{$\ket{0}^{\otimes m}$} \\
& \push{\rvdots}\wireoverride{n} & \wireoverride{n} & \wireoverride{n} & \wireoverride{n}  & \wireoverride{n} & \wireoverride{n} & \wireoverride{n} & \wireoverride{n} & \wireoverride{n} & \wireoverride{n}\\
& \qw & \qw & \gate{P(-\frac{\gamma_1}{2^{m}})} & \qw & \qw & \qw & \ \ldots\ & \qw & \qw & \\
\lstick{$\ket{0}^{\otimes a}$} & \qw & \gateinput[1]{$0$}\gateoutput[1]{$*$} & \qw & \qw & \midstick[1]{$\ket{0}^{\otimes a}$} & \qw & \ \ldots\ & \qw & \qw &\rstick{$\ket{0}^{\otimes a}$}
\end{quantikz}%\octrl{0}\wire[l][1]["\beta_1"{above, pos=-0.3}]{a}

==> tikz/quso-structure.tex <==
\begin{tikzpicture}
\node[draw] at (0,0) {1. QSim using QDAC $\ket{x}\ket{0}^{\otimes a} \mapsto \ket{x}\ket{y}$, 2. SSIX $\mathcal{H}\rightarrow \left[-0.5,0.5\right[$, 3. QADC via QPA};
\end{tikzpicture}

==> tikz/x-in_dep-CQSP-combined.tex <==
\begin{quantikz}[column sep=5.3pt, row sep={25pt,between origins}]
\lstick{$\ket{0}$} & \gate{H} & \octrl{1} & \ctrl{2} & \rstick[3]{$\quad\begin{pmatrix}
           \ket{b}/\sqrt{2} \\
           \ket{c(x)}/\sqrt{2} \\
           0\\
         \end{pmatrix}$} \\
\lstick{$\ket{0}^{\otimes n-m}$}  & \qw & \gate[disable auto height]{U_b} & \qw &   \rstick{}\\
\lstick{$\ket{0}^{\otimes m}$}  & \qw & \qw & \gate[disable auto height]{U_c} & \rstick{}
\end{quantikz}

==> txt/6-Conclusion.tex <==
\begin{itemize}
    \item Exponential speedup possible for many use cases (classical runtime usually as large as needed to even properly describe the problem)
    \item Close investigation needed for all potential use cases in regards to: classical runtime complexity for setup of the systems of linear equations, condition number and quantum implementation of the calculation of the cost from the solution vector 
    \item Qubit requirements can be traded off with runtime, but also efficient oracles for structured problems should be investigated
    \item Practical limits: QSP Phase angles!! Maybe the solution: Mapping the existing ideas of GQSP to ``GQSVT''.
\end{itemize}
